J-PLUS Tracking Tool: Scheduler and Tracking software for the Observatorio Astrof\'isico de Javalambre (OAJ)

The Javalambre Photometric Local Universe Survey (J-PLUS) is an ongoing 12 band photometric optical survey, observing thousands of square degrees of the Northern Hemisphere from the dedicated JAST80 telescope at the Observatorio Astrof\'isico de Javalambre (OAJ). Observational strategy is a critical point in this large survey. To plan the best observations, it is necessary to select pointings depending on object visibility, the pointing priority and status and location and phase of the Moon. In this context, the J-PLUS Tracking Tool, a web application, has been implemented, which includes tools to plan the best observations, as well as tools to create the command files for the telescope; to track the observations; and to know the status of the survey. In this environment, robustness is an important point. To obtain it, a feedback software system has been implemented. This software automatically decides and marks which observations are valid or which must be repeated. It bases its decision on the data obtained from the data management pipeline database using a complex system of pointing and filter statuses. This contribution presents J-PLUS Tracking Tool and all feedback software system.

==> Makefile <==
# Example makefile to help you compile your ADASS proceedings
# but you really should read the ManuscriptInstructions.pdf or
# at least the README file. For some smart cookies the Makefile
# could be sufficient too.
#
# Version 7-oct-2022   Peter Teuben & Severin Gaudet
#
# See also:   https://www.adass2022.ca/.... / ADASS2022.tar
#
# P = paper_id    your proceedings paper ID code (the one with the XNN syntax, e.g., O12)
# V = version     your version # (1,2,..) since you can only upload unique files
# A = 1stauthor   your last name, e.g. Teuben
# E = email       your contact email for submission issues
# FIGS = *eps     your EPS figures

                    # put your paper_id here (with dash, not dot), e.g. P10-2
                    # or find your template on http://www.astro.umd.edu/~teuben/adass/papers/
P = $(shell detect_tex.py | grep -v '^%' | sed 's/.tex//g')
                    # keep incrementing this after each upload of your $(P)
V = 1
                    # First author (for Papercheck.py)
A = Teuben
                    # contact person email
E = teuben@gmail.com
		    # your EPS figures (can be blank, and must be base-named with $(P)_*.eps
FIGS = $(shell ls *.eps)

# override P,V,A,E,FIGS with a "makedefs" file, this is where authors should edit, not this Makefile
-include makedefs

# Which command do you use to view the PDF? This is just for convenience.
# PDFOPEN = xdg-open
PDFOPEN = open

#  variables for proceeding editors (don't modify, for export, not for authors)
YEAR   = 2022
ATDIR  = ADASS$(YEAR)_author_template
FILES  = AdassChecks.py AdassConfig.py AdassIndex.py ADASS_template.tex \
	 Aindex.py FixUnprintable.py \
	 copyrightform.pdf example.bib example.eps \
	 Index.py manual2010.pdf ManuscriptInstructions.pdf PaperCheck.py \
	 README subjectKeywords.txt TexScanner.py \
	 ascl.py asclKeywords.txt \
	 adass$(YEAR).bib Makefile makedefs.example \
	 $(FILESASP)

#  probably don't change these either (or notify the editors you have a special paper case)
PID_URL   = "https://www.canfar.net/storage/vault/list/adass2022/upload/$(P)"
TAR_FILE  = $(P).tar.gz
ZIP_FILE  = $(P).zip
POS_FILE  = $(P).pdf
FILESPDF  = $(P).pdf copyrightForm_$(P)_$(A).pdf
FILESTEX  = $(P).tex $(P).bib $(FIGS) makedefs
FILESASP  = asp2014.bst asp2014.sty
FILES4AR  = $(FILESTEX) $(FILESPDF)

# ensure current directory is in the PATH
export PATH := .:$(PATH)

help:
	@echo AUTHOR targets:
	@echo ---------------
	@echo all:   pdf check tar
	@echo pdf:
	@echo check:
	@echo clean:
	@echo overleaf:
	@echo tar:
	@echo zip:
	@echo 
	@echo EDITOR targets:
	@echo ---------------
	@echo fix:
	@echo inc:
	@echo spell:
	@echo aindex:
	@echo words:
	@echo asp1:
	@echo index:   needs TERMS=
	@echo ascl:
	@echo ascl1:
	@echo ascl2:   needs CODE=
	@echo pdf2:
	@echo rsync:


all:	pdf check tar


# not for authors, for creator of the ADASS instruction tar file
export:
	rm -rf $(ATDIR)
	mkdir  $(ATDIR)
	cp -a $(FILES) $(ATDIR)
	echo Created on `date` by `whoami`  > $(ATDIR)/VERSION
	-git remote -v                     >> $(ATDIR)/VERSION
	-git branch                        >> $(ATDIR)/VERSION
	tar cf ADASS$(YEAR).tar $(ATDIR)

# copyright is now part of the tar/zip file, checksum (sum) is 13785
copyrightForm_$(P)_$(A).pdf: copyrightform.pdf
	cp copyrightform.pdf copyrightForm_$(P)_$(A).pdf
	@echo Now go edit your copyrightForm_$(P)_$(A).pdf form

# these targets are for most common unix systems, but YMMV. Modify if you need
# let the editors know you have a better way for the next ADASS team
# ASP prefers the latex;latex;dvipdfm route

DVIPDF = dvipdf

pdf:	$(P).pdf
	@echo $(PDFOPEN) $(P).pdf 

$(P).pdf:  $(P).dvi $(FIGS)
	$(DVIPDF) $(P)

$(P).bib:                                  # bootstrap if you don't have one
	touch $(P).bib

$(P).dvi:  $(P).tex $(P).bib
	latex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	latex $(P)
	latex $(P)

# an alternative method (ASP does not recommend it)
pdflatex:
	pdflatex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	pdflatex $(P)
	pdflatex $(P)

clean:
	rm -f $(P).dvi $(P).bbl $(P).blg $(P).pdf $(P).aux $(P).log $(P).out $(P).toc $(P)_inc.tex

check:
	PaperCheck.py $(P) $(A)

ENCODING =
fix:
	FixUnprintable.py  $(P).tex $(ENCODING)

inc:
	tex2inc.py $(P).tex > $(P)_inc.tex
	@tail -1 $(P)_inc.tex
	@cat $(P).toc

spell:
	aspell --mode=tex --lang=en check $(P).tex
	@echo Share your ~/.aspell.en.pws  ~/.aspell.en.prepl

aspell:
	(cd ../..; $(MAKE) aspell)

dvi:
	latex $(P)

aindex:
	Aindex.py $(P)

DETEX = detex
words:
	$(DETEX) $(P).tex | grep -o -E '\w+' | tr '[A-Z]' '[a-z]' | sort | uniq -c | sort -n

#  could add a checksum on personal copyrightform - if it's 13785,it's bad.
tar:    $(FILES4AR) _checksum
	tar zcf $(TAR_FILE) $(FILES4AR)
	@echo "Login and upload $(TAR_FILE) at $(PID_URL)"

zip:    $(FILES4AR) _checksum
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILES4AR)
	@echo "Login and upload $(ZIP_FILE) at $(PID_URL)"

poster: $(POS_FILE)
	@echo "Login and upload $(POS_FILE) at $(PID_URL)"

overleaf:    $(FILESTEX)
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILESTEX) $(FILESASP)
	@echo You can now upload $(ZIP_FILE) as a new project into overleaf
	@echo After import, git clone this here, and move all the git tree files here.
	@echo "The git clone command is under overleaf's Menu"


_checksum: copyrightForm_$(P)_$(A).pdf
	@echo Checksum test
	@sum copyrightForm_$(P)_$(A).pdf

# for editors
asp1:
	(cd ../..; $(MAKE) asp1 PID=$(P); grep box asp1.log)
	@echo $(PDFOPEN) ../../authors/$(P).pdf

TERMS = foobar
index:
	@echo Using TERMS=$(TERMS)
	(cd ../Author_Template; Index.py $(TERMS))

ssindex:
	@echo Generating ssindex list
	(cd ../Author_Template; ssindex-org.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ssindex2:
	@echo Generating scored ssindex list 
	(cd ../Author_Template; ssindex-scored.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

index2:
	(cd ../adass_subject_recommender ; detex ../$(P)/$(P).tex |  PYTHONPATH=`pwd` bin/find_subjects.py -m 10 -j)

ascl:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)
# 	(cd ../Author_Template; ascl-new.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ascl1:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex | grep ooindex | sort | uniq -c)
	-detex $(P).tex > $(P).txt
	-(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).txt | grep ooindex | sort | uniq -c)
	-grep ooindex $(P).tex

CODE = foobar
.PHONY: ascl2
ascl2:
	$(PDFOPEN) https://ascl.net/$(CODE)

pdf2:   pdf asp1
	$(PDFOPEN) $(P).pdf
	$(PDFOPEN) ../../authors/$(P).pdf

rsync: $(P).bib
	rsync -av $(P)_inc.tex $(P).bib $(FIGS) ../../authors
	rm -f ../../authors/$(P)_inc.{bbl,blg}


